IDT: Dual-Task Adversarial Attacks for Privacy Protection

Natural language processing (NLP) models may leak private information in different ways, including membership inference, reconstruction or attribute inference attacks. Sensitive information may not be explicit in the text, but hidden in underlying writing characteristics. Methods to protect privacy can involve using representations inside models that are demonstrated not to detect sensitive attributes or -- for instance, in cases where users might not trust a model, the sort of scenario of interest here -- changing the raw text before models can have access to it. The goal is to rewrite text to prevent someone from inferring a sensitive attribute (e.g. the gender of the author, or their location by the writing style) whilst keeping the text useful for its original intention (e.g. the sentiment of a product review). The few works tackling this have focused on generative techniques. However, these often create extensively different texts from the original ones or face problems such as mode collapse. This paper explores a novel adaptation of adversarial attack techniques to manipulate a text to deceive a classifier w.r.t one task (privacy) whilst keeping the predictions of another classifier trained for another task (utility) unchanged. We propose IDT, a method that analyses predictions made by auxiliary and interpretable models to identify which tokens are important to change for the privacy task, and which ones should be kept for the utility task. We evaluate different datasets for NLP suitable for different tasks. Automatic and human evaluations show that IDT retains the utility of text, while also outperforming existing methods when deceiving a classifier w.r.t privacy task.

==> 8_limitations.tex <==
\section{Limitations}

The \attack attack finds words to replace based on their importance for two tasks. This, coupled with the tight constraint of ensuring equal POS tags between all adversarial and original tokens, limits the amount of candidate adversarial sentences it can generate, compared to baselines which look at only one task, as Table \ref{tab:attacks_generated_sentences} in the Appendix shows.


In addition, even though TOEFL11 is a standard dataset for native language identification, it is a proprietary one and therefore it cannot be freely shared (although it is available under standard conditions through the Linguistic Data Consortium). We note, though, that the other datasets we used are publicly available.

Finally, despite our extensive quality assessment of the adversarial texts with automatic measurements, we do not present human evaluation on how \attack compares against baselines w.r.t. attributes such as fluency, correctness or naturalness from a human point of view; as evidenced in \citet{dyrmishi-etal-2023-humans}, knowing what is the best kind of human evaluation for these minimally perturbed text is question that is still being explored.

%\section{Ethics Statement}  

%The authors declare no conflict of interest. We also note that all datasets we used have been widely used in the literature and were collected with the purpose of scientific research. We acknowledge the risks posed by adversarial attacks, but we also consider that they can be helpful in enhancing privacy as in the scenarios outlined by this paper.

==> pfgplotsres.tex <==
Figure \ref{fig:attack_results} brings the 

\begin{figure*}[t]
    \centering
    \subfloat[TOEFL11\textsubscript{S}]{%
        \begin{tikzpicture}
            \begin{axis}[
                ybar,
                bar width=0.4cm,
                width=0.5\textwidth, % Adjust the width of the figure
                height=6cm, % Adjust the height of the figure
                ylabel={\%},
                %xlabel={Categories},
                symbolic x coords={IDT, TextFooler, TextBugger, BAE},
                xtick=data,
                %legend style={at={(0.5,-0.15)}, anchor=north, legend columns=-1},
                ]
                \addplot[fill=blue!30] coordinates {(IDT, 44.85) (TextFooler, 42.93) (TextBugger, 43.46) (BAE, 6)};
                \addplot[fill=red!30] coordinates {(IDT, 97.16) (TextFooler, 95.25) (TextBugger, 96.94) (BAE, 7)};
                \legend{AS, UR}
            \end{axis}
        \end{tikzpicture}%
    }%
    \hfill
    \subfloat[TOEFL11\textsubscript{C}]{%
        \begin{tikzpicture}
            \begin{axis}[
                ybar,
                bar width=0.4cm,
                width=0.5\textwidth, % Adjust the width of the figure
                height=6cm, % Adjust the height of the figure
                ylabel={\%},
                %xlabel={Categories},
                symbolic x coords={IDT, TextFooler, TextBugger, BAE},
                xtick=data,
                %legend style={at={(0.5,-0.15)}, anchor=north, legend columns=-1},
                ]
                \addplot[fill=blue!30] coordinates {(IDT, 29.6) (TextFooler, 32.25) (TextBugger, 31.13) (BAE, 6)};
                \addplot[fill=red!30] coordinates {(IDT, 98.93) (TextFooler, 99.13) (TextBugger, 99.32) (BAE, 7)};
                \legend{AS, UR}
            \end{axis}
        \end{tikzpicture}%
    }%
    \hfill
    \subfloat[Shakespeare]{%
        \begin{tikzpicture}
            \begin{axis}[
                ybar,
                bar width=0.4cm,
                width=0.5\textwidth, % Adjust the width of the figure
                height=6cm, % Adjust the height of the figure
                ylabel={\%},
                %xlabel={Categories},
                symbolic x coords={IDT, TextFooler, TextBugger, BAE},
                xtick=data,
                %legend style={at={(0.5,-0.15)}, anchor=north, legend columns=-1},
                ]
                \addplot[fill=blue!30] coordinates {(IDT, 68.12) (TextFooler, 46.26) (TextBugger, 47.74) (BAE, 6)};
                \addplot[fill=red!30] coordinates {(IDT, 85.31) (TextFooler, 71.49) (TextBugger, 75.11) (BAE, 7)};
                \legend{AS, UR}
            \end{axis}
        \end{tikzpicture}%
    }%
    \subfloat[TrustPilot]{%
        \begin{tikzpicture}
            \begin{axis}[
                ybar,
                bar width=0.4cm,
                width=0.5\textwidth, % Adjust the width of the figure
                height=6cm, % Adjust the height of the figure
                ylabel={\%},
                %xlabel={Categories},
                symbolic x coords={IDT, TextFooler, TextBugger, BAE},
                xtick=data,
                %legend style={at={(0.5,-0.15)}, anchor=north, legend columns=-1},
                ]
                \addplot[fill=blue!30] coordinates {(IDT, 45.44) (TextFooler, 32.25) (TextBugger, 31.13) (BAE, 6)};
                \addplot[fill=red!30] coordinates {(IDT, 99.89) (TextFooler, 99.13) (TextBugger, 99.32) (BAE, 7)};
                \legend{AS, UR}
            \end{axis}
        \end{tikzpicture}%
    }%
    \caption{\textit{Attak Success} (\textbf{AS}) and \textit{Utility Retention} (\textbf{UR}) for each dataset under different attacks.}
    \label{fig:attack_results}
\end{figure*}
